Learning to Contextually Aggregate Multi-Source Supervision for Sequence Labeling

Sequence labeling is a fundamental framework for various natural language processing problems. Its performance is largely influenced by the annotation quality and quantity in supervised learning scenarios, and obtaining ground truth labels is often costly. In many cases, ground truth labels do not exist, but noisy annotations or annotations from different domains are accessible. In this paper, we propose a novel framework Consensus Network (ConNet) that can be trained on annotations from multiple sources (e.g., crowd annotation, cross-domain data...). It learns individual representation for every source and dynamically aggregates source-specific knowledge by a context-aware attention module. Finally, it leads to a model reflecting the agreement (consensus) among multiple sources. We evaluate the proposed framework in two practical settings of multi-source learning: learning with crowd annotations and unsupervised cross-domain model adaptation. Extensive experimental results show that our model achieves significant improvements over existing methods in both settings. We also demonstrate that the method can apply to various tasks and cope with different encoders.

==> sections/5_exp_update.tex <==
\section{Experiments}


\begin{table*}[thbp]
\centering
\scalebox{0.7}{
\begin{tabular}{lcccccc}
    \toprule  
    \multirow{2}{*}{\textbf{Methods}}&
    \multicolumn{3}{c}{ \textbf{AMTC}}&\multicolumn{3}{c}{ \textbf{AMT}}\\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & Precision(\%) & Recall(\%) & F1-score(\%) & Precision(\%) & Recall(\%) & F1-score(\%)  \\
    \midrule  
    {CONCAT-SLM}  &  \textbf{85.95}($\pm$1.00)  &  57.96($\pm$0.26)  &  69.23($\pm$0.13) & \textbf{91.12}($\pm$0.57) & 55.41($\pm$2.66) & 68.89($\pm$1.92) \\
    {MVT-SLM}  &  84.78($\pm$0.66)  &  62.50($\pm$1.36)  &  71.94($\pm$0.66) & 86.96($\pm$1.22) & 58.07($\pm$0.11) & 69.64($\pm$0.31) \\
    {MVS-SLM} &  84.76($\pm$0.50)  &  61.95($\pm$0.32)  &  71.57($\pm$0.04) & 86.95($\pm$1.12) & 56.23($\pm$0.01) & 68.30($\pm$0.33) \\
    {DS-SLM}~\citep{Nguyen2017ACL}  &  72.30$^*$  &  61.17$^*$  &  66.27$^*$ & - & - & - \\
    {HMM-SLM}~\citep{Nguyen2017ACL} &  76.19$^*$  &  66.24$^*$  &  70.87$^*$ & - & - & - \\
    {MTL-MVT}~\citep{Wang2018BioNER}  & 81.81($\pm$2.34) & 62.51($\pm$0.28) & 70.87($\pm$1.06) &  88.88($\pm$0.25)  & 65.04($\pm$0.80)   & 75.10($\pm$0.44)   \\
    {MTL-BEA}~\citep{rahimi2019massively} & 85.72($\pm$0.66) & 58.28($\pm$0.43) & 69.39($\pm$0.52) & 77.56($\pm$2.23) & 67.23($\pm$0.72) & 72.01($\pm$0.85) \\
    \midrule
    {CRF-MA}~\citep{Rodrigues2014ML} & 49.40$^*$  &  85.60$^*$  &  62.60$^*$ &  49.40$^*$  &  85.60$^*$  &  62.60$^*$  \\
    {Crowd-Add}~\citep{Nguyen2017ACL}  &  85.81($\pm$1.53)  &  62.15($\pm$0.18)  &  72.09($\pm$0.42) & 89.74($\pm$0.10) & 64.50($\pm$1.48) & 75.03($\pm$1.02) \\
    {Crowd-Cat}~\citep{Nguyen2017ACL}  & 85.02($\pm$0.98) & 62.73($\pm$1.10) & 72.19($\pm$0.37) &  89.72($\pm$0.47) & 63.55($\pm$1.20) & 74.39($\pm$0.98) \\
    {CL-MW}~\citep{Rodrigues2018AAAI}  & - & - & - &  66.00$^*$  &  59.30$^*$  &  62.40$^*$  \\
    \midrule
    \textsc{ConNet} (Ours) &  84.11($\pm$0.71)  &  \textbf{68.61}($\pm$0.03)  &  \textbf{75.57}($\pm$0.27) & 88.77($\pm$0.25) & \textbf{72.79}($\pm$0.04) & \textbf{79.99}($\pm$0.08) \\
    \midrule
    {Gold} (Upper Bound) &  89.48($\pm$0.32)  &  89.55($\pm$0.06)  &  89.51($\pm$0.21) & 92.12($\pm$0.31) & 91.73($\pm$0.09) & 91.92($\pm$0.21) \\
    \bottomrule 
\end{tabular}
}
\caption{\small{Performance on real-world crowd-sourced NER datasets.
(* indicates number reported by the paper.)}
}
\label{tab:res:real}
\end{table*}

We evaluate \textsc{ConNet} in two practical settings of multi-source learning: learning with crowd annotations and unsupervised cross-domain model adaptation. In the crowd annotation learning setting, the training data of the same domain is annotated by multiple noisy annotators. In the decoupling phase, the model is trained on noisy annotations, and in the aggregation phase, it is trained with combined predictions on the training set. In the cross-domain setting, the model has access to unlabeled training data of the target domain and clean labeled data of multiple source domains. In the decoupling phase, the model is trained on source domains, and in the aggregation phase, the model is trained on combined predictions on the training data of the target domain. 

In addition to BLSTM-CRF, our framework can potentially generalize to other encoders. Therefore we also test our method on text classification with an MLP encoder. In this setting, hidden representations of MLP are transformed by multiplying crowd/consensus matrices and the transformed representation is then used by a classification layer to make predictions.

\subsection{Datasets}
\label{sec:exp:data}

\textbf{Crowd-Annotation Datasets.}
We use crowd-annotation datasets based on the 2003 CoNLL shared NER task ~\citep{tjong-kim-sang-de-meulder-2003-introduction}. The real-world datasets, denoted as AMT, are collected by~\citet{Rodrigues2014ML} using Amazon's Mechanical Turk where F1 scores of annotators against the ground truth vary from 17.60\% to 89.11\%. Since there is no development set in AMT, we also follow~\citet{Nguyen2017ACL} to use the AMT training set and CoNLL 2003 development and test sets, denoted as AMTC. Overlapping sentences are removed in the training set, which is ignored in that work. 
Additionally, we construct two sets of simulated datasets to investigate the quality and quantity of annotators. To simulate the behavior of a non-expert annotator, a CRF model is trained on a small subset of training data and generates predictions on the whole set. Because of the limited size of training data, each model would have a bias to certain patterns.

\textbf{Cross-Domain Datasets.}
In this setting, we investigate three NLP tasks: POS tagging, NER and text classification.
%We consider the Universal Dependencies (UD) v2.3 corpus~\citep{nivre2016universal} for multi-domain POS tagging. The GUM portion~\citep{zeldes2017gum} of the corpus is used because it has relatively balanced data for each domain. 
For POS tagging task, we use the GUM portion~\citep{zeldes2017gum} of Universal Dependencies (UD) v2.3 corpus with $17$ tags and $7$ domains: academic, bio, fiction, news, voyage, wiki, and interview. 
For NER task, we select the English portion of the OntoNotes v5 corpus~\citep{hovy2006ontonotes}. The corpus is annotated with $9$ named entities with data from $6$ domains: broadcast conversation (bc), broadcast news (bn), magazine (mz), newswire (nw), pivot text (pt), telephone conversation (tc), and web (web). 
Multi-Domain Sentiment Dataset (MDS) v2.0~\citep{blitzer2007biographies} is used for text classification, which is built on Amazon reviews from $4$ domains: books, dvd, electronics, and kitchen. Since the dataset only contains word frequencies for each review without raw texts, we follow the setting in~\citet{chen-cardie-2018-multinomial} considering 5,000 most frequent words and use the raw counts as the feature vector for each review.

\subsection{Experiment Setup}
\label{sec:exp:setup}

For sequence labeling tasks, we follow \citet{liu2018efficient} to build the BLSTM-CRF architecture as the base model. The dimension of character-level, word-level embeddings and BLSTM hidden layer are set as $30$, $100$ and $150$ respectively.
For text classification, each review in the MDS dataset is represented as a $5000$-d feature vector. We use an MLP with a hidden size of $100$ for encoding such features and a linear classification layer for predicting their labels.
The dropout with a probability of $0.5$ is applied to the non-recurrent connections for regularization.
The network parameters are randomly initialized and updated by stochastic gradient descent (SGD).
The learning rate is initialized as $0.015$ and decayed by $5\%$ for each epoch.
The training process stops early if no improvements in $15$ continuous epochs and selects the best model on the development set.
For the dataset without a development set, we report the performance on the $50$-th epoch.
For each experiment, we report the average performance and standard variance of $3$ runs with different random initialization.

\subsection{Comparison with Baseline Methods}
\label{sec:exp:comp}

We compare our models with multiple baselines, which can be categorized in two groups: wrapper methods and joint models. To demonstrate the theoretical upper bound of performance, we also train the base model using ground-truth annotations in the target domain (\texttt{Gold}).

A wrapper method consists of a label aggregator and a deep learning model. These two components could be combined in two ways: (1) aggregating labels on crowd-sourced training set then feeding the generated labels to a Sequence Labeling Model (\texttt{SLM})~\citep{Liu2017EMNLP}; (2) feeding multi-source data to a Multi-Task Learning (\texttt{MTL})~\citep{Wang2018BioNER} model then aggregating multiple predicted labels. 
We investigate multiple label aggregation strategies. \texttt{CONCAT} considers all crowd annotations as gold labels. \texttt{MVT} does majority voting on the token level, \ie, the majority of labels $\{\by_{i,j}^k\}$ is selected as the gold label for each token $\bx_{i,j}$. \texttt{MVS} is conducted on the sequence level, addressing the problem of violating Begin/In/Out (BIO) rules. \texttt{DS}~\citep{Dawid1979EM}, \texttt{HMM}~\citep{Nguyen2017ACL} and \texttt{BEA}~\citep{rahimi2019massively} induce consensus labels with probability models.

In contrast with wrapper methods, joint models incorporate multi-source data within the structure of sequential taggers and jointly model all of the individual annotators. \texttt{CRF-MA} models CRFs with Multiple Annotators by EM algorithm~\citep{Rodrigues2014ML}.
\citet{Nguyen2017ACL} augments the LSTM architecture with crowd vectors.
These crowd components are element-wise added to the tags scores (\texttt{Crowd-Add}) or concatenated to the output of the hidden layer (\texttt{Crowd-Cat}).
These two methods are the most similar to our extraction phase. We implemented them and got better results than reported.
\texttt{CL-MW} applies a crowd layer to a CNN-based deep learning framework \citep{Rodrigues2018AAAI}. 
\texttt{Tri-Training} uses bootstrapping with multi-task Tri-Training approach for unsupervised one-to-one domain adaptation~\citep{saito2017asymmetric,ruder-plank-2018-strong}. 

\subsection{Learning with Crowd Annotations}

\begin{table}[htbp]
    \centering
    %\begin{tabular}{|c|p{12.5cm}|}
    \begin{tabular}{|c|m{0.9\columnwidth}|}
    %\hline
    %index & sentence \\
    \hline
        1 & Defender \PER{Hassan Abbas} rose to intercept a long ball into the area in the 84th minute but only managed to divert it into the top corner of \PER{Bitar} 's goal . \\
        \hline
        2 & \ORG{Plymouth} 4 \ORG{Exeter} 1 \\
        \hline
        3 & Hosts \LOC{UAE} play \LOC{Kuwait} and \LOC{South Korea} take on \LOC{Indonesia} on Saturday in Group A matches . \\
        \hline
        4 & The former \MISC{Soviet} republic was playing in an \MISC{Asian Cup} finals tie for the first time . \\
        \hline
        5 & \PER{Bitar} pulled off fine saves whenever they did . \\ \hline
        6 & \PER{Coste} said he had approached the player two months ago about a comeback . \\ \hline
        7 & \ORG{Goias} 1 \ORG{Gremio} 3 \\ \hline
        8 & \ORG{Portuguesa} 1 \ORG{Atletico Mineiro} 0 \\ \hline
        9 & \LOC{Melbourne} 1996-12-06 \\ \hline
        10 & On Friday for their friendly against \LOC{Scotland} at \LOC{Murrayfield} more than a year after the 30-year-old wing announced he was retiring following differences over selection . \\ \hline
        11 & Scoreboard in the \MISC{World Series} \\ \hline
        12 & Cricket - \MISC{Sheffield Shield} score . \\ \hline
        13 & `` He ended the \MISC{World Cup} on the wrong note , " \PER{Coste} said . \\ \hline
        14 & Soccer - \ORG{Leeds} ' \PER{Bowyer} fined for part in fast-food fracas . \\ \hline
        15 & \ORG{Rugby Union} - \PER{Cuttitta} back for \LOC{Italy} after a year . \\ \hline
        16 & \LOC{Australia} gave \PER{Brian Lara} another reason to be miserable when they beat \LOC{West Indies} by five wickets in the opening \MISC{World Series} limited overs match on Friday . \\ 
        \hline
    \end{tabular}
    \caption{Sample instances in Fig.~\ref{fig:exp:crowd:caseheat} with NER annotations including \texttt{PER} (red), \texttt{ORG} (blue), \texttt{LOC} (violet) and \texttt{MISC} (orange).}
    \label{tab:exp:crowd:cases}
\end{table}

\subsubsection{Performance on real-word datasets}

Tab.~\ref{tab:res:real} shows the performance of aforementioned methods and our \textsc{ConNet} on two real-world datasets, \ie~AMT and AMTC\footnote{\scriptsize We tried our best to re-implement the baseline methods for all datasets, and left the results blank when the re-implementation is not showing consistent results as in the original papers.}.
We can see that \textsc{ConNet} outperforms all other methods on both datasets significantly on $F1$ score, which shows the effectiveness of dealing with noisy annotations for higher-quality labels.
Although \texttt{CONCAT-SLM} achieves the highest precision, it suffers from low recall.
All existing methods have the high-precision but low-recall problem.
One possible reason
is that they try to find the latent ground truth and throw away illuminating annotator-specific information. 
So only simple mentions can be classified with great certainty while difficult mentions fail to be identified without sufficient knowledge.
In comparison, \textsc{ConNet} pools information from all annotations and focus on matching knowledge to make predictions. 
It makes the tagging model be able to identify more mentions and get a higher recall.


%%%%%%%%%%%%%
%% case study
%%%%%%%%%%%%%
\subsubsection{Case Study}
\label{sec:app:ab}
It is enlightening to analyze whether the model decides the importance of annotators given a sentence. In Fig.~\ref{fig:exp:crowd:caseheat} we visualize normalized expertise over all annotators, and attention weights $\bq_i$ in Eq.~\ref{eq:attvec} for $16$ sampled sentences containing different entity types. Sentence 1-12 contains a specific entity type respectively while 13-16 contains multiple different entities. Details are described in Tab.~\ref{tab:exp:crowd:cases}. Compared with expertise of annotators, we can see that the attention module would give more weight on annotators who have competitive performance and preference on the included entity type. Although top selected annotators for \texttt{ORG} has relatively lower expertise on \texttt{ORG} than \texttt{PER} and \texttt{LOC}, they are actually the top three annotators with highest expertise on \texttt{ORG}. Obviously, the $2$nd sample sentence with \texttt{ORG} has higher attention weights on $1$st, $5$th and $33$rd annotator who are best at labeling \texttt{ORG}.

%%%%%%%%%%%%%
%% ablation study
%%%%%%%%%%%%%
\subsubsection{Ablation Study}
\label{sec:app:ab}

\begin{figure}[htbp]
\centering
    
    \includegraphics[width=0.9\linewidth]{figures/exp/crowdsource/res_ab.png}
\caption{Performance of \textsc{ConNet} variants for ablation study.}
\label{fig:exp:crowd:ab}
\end{figure}

To investigate the effectiveness of our proposed method, multiple variants of the decoupling phase and aggregation phase are evaluated on the AMT dataset, shown in Fig.~\ref{fig:exp:crowd:ab}.

\noindent \textbf{Decoupling Phase}
We tried three different approaches to incorporate source-specific representation in the decoupling phase (DP). \texttt{CRF} means the traditional approach without annotator matrices as Eq.~\ref{eq:crf} while \texttt{DP(1+2)} is described in Eq.~\ref{eq:df:crf}. Similarly, \texttt{DP(1)} only applies source representations $\bA^{(k)}$ to the emission score $\bU$ while \texttt{DP(2)} only transfers the transition matrix $\bM$.
They directly use latent representations $\bU$ and $\bM$ in the decoupling phase (not augmented by $\bA^{(k)}$) for prediction.
We can observe from the result that both variants that model the annotator-specific information can improve the result.
The underlying model keeps more consensus knowledge if we extract annotator-specific bias on sentence encoding and label transition.

\noindent \textbf{Aggregation Phase} We compare four methods of generating supervision targets in the aggregation phase (AP). 
%These methods are illustrated in Fig.~\ref{fig:exp:crowd:simu:ab}(right) , and they all use the same extraction phase as {(1+2)}. 
\texttt{OMV} uses majority voting of original annotations as targets for training, while \texttt{PMV} substitutes them with model prediction learned from DP. \texttt{AMV} extends the model by using all prediction, while \texttt{AWV} uses majority voting weighted by each annotator's training $F1$ score.
The results show the effectiveness of \texttt{AWV}, which could well approximate the ground truth and supervise the attention module to estimate the expertise of annotator on the current sentence.
We can also infer labels on the test set by conducting \texttt{AWV} on predictions of the underlying model with each annotator-specific components.
But it leads to heavy computation-consuming and unsatisfying performance, whose test $F1$ score is $77.35(\pm 0.08)$.
To investigate the importance of extracted source-specific components, we trained a traditional BLSTM-CRF model by the supervision of the same \texttt{AMV} labels.
Its result is $78.93(\pm 0.13)$, which is lower than our \textsc{ConNet}. 

These experiments convey four messages: 
(1) Using learned model prediction is better than directly using original annotations as its target; 
(2) It is desirable to use all model predictions instead of just confine each annotator on their data set. This means that the learned representation of individual annotator can generalize on data it didn't annotate. 
(3) Weighting aggregating models by their performance is beneficial to overall accuracy.
(4) The attention model could learn to estimate annotators' ability based on the context. 

\begin{figure}
\vspace{-0.2cm}
\centering  
    \subfigure{
    \label{fig:exp:crowd:simu:real}
    \includegraphics[width=0.8\linewidth]{figures/exp/crowdsource/res_simu_real.pdf}}
\subfigure{
    \label{fig:exp:crowd:simu:num}
    \includegraphics[width=0.8\linewidth]{figures/exp/crowdsource/res_simu_num.pdf}}
    % \includegraphics[width=.9\linewidth]{figures/exp/crowdsource/res_simu.pdf}
    \vspace{-0.4cm}
\caption{\small Performance on simulated crowd-sourced NER datasets with (a) $5$ annotators on different reliability levels; (b) various numbers of annotators whose reliability $r=1/50$. 
% \vspace{-0.2cm}
 }
\label{fig:exp:crowd:simu}
\end{figure}

\subsubsection{Analysis of Annotators Impact}
To analyze the impact of annotator quality, we split the origin train set into $\{5, 10, 15, 30, 50\}$ folds and train a CRF model on each fold whose reliability could be represented as $r=\{1/5, 1/10, 1/15, 1/30, 1/50\}$ because a model with less training data would have stronger bias and less generalization. For each setting, we randomly select $5$ trained models as the simulated annotators. When the reliability level of all annotators is too low, \ie~$1/50$, only the base model is used for prediction without annotator representations.
Shown in Fig.~\ref{fig:exp:crowd:simu}(a), \textsc{ConNet} achieves significant improvements over \texttt{MVT-SLM} and competitive performance as \texttt{Crowd-Cat}. Our model shows its effectiveness when annotators are less reliable.

Regarding the influence of annotator quantity, we split the train set into $50$ subsets to train $50$ models ($r=1/50$) respectively and randomly select $\{5, 10, 15, 30, 50\}$ models as simulated annotators.
Fig.~\ref{fig:exp:crowd:simu}(b) shows \textsc{ConNet} is superior to baselines and able to well deal with many annotators while there is no obvious relationship between the performance and the number of annotators in baselines. 

\begin{figure*}
\vspace{-0.4cm}
    \centering
    \includegraphics[width=1.95\columnwidth]{figures/exp/crowdsource/csheat.pdf}
    % \vspace{-0.2cm}
    \caption{\small Visualizations of (a) the expertise of annotators; (b) attention weights for sample sentences.
    \vspace{-0.5cm}
    }
    \label{fig:exp:crowd:caseheat}
\end{figure*}

\subsection{Cross-Domain Adaptation}

\begin{table*}[htbp]
\centering
\scalebox{0.76}{
\begin{tabularx}{1.3\textwidth}{l|c c c c c c c|l}
  \toprule
  Task \& Corpus & \multicolumn{8}{c}{\bf Multi-Domain POS Tagging: Universal Dependencies v2.3 - GUM} \\
  \midrule
  Target Domain & academic & bio~~ & ~fiction~ & ~~news~ & voyage~ & wiki & interview & AVG $Acc$(\%) \\
  \midrule
  CONCAT & 92.68 & 92.12 & 93.05 & 90.79 & 92.38 & 92.32 & 91.44 & 92.11($\pm$0.07) \\
  MTL-MVT~\citep{Wang2018BioNER} & 92.42 & 90.59 & 91.16 & 89.69 & 90.75 & 90.29 & 90.21 & 90.73($\pm$0.29) \\
  MTL-BEA~\citep{rahimi2019massively} & 92.87 & 91.88 & 91.90 & 91.03 & 91.67 & 91.31 & 91.29 & 91.71($\pm$0.06) \\
  \midrule
  Crowd-Add~\citep{Nguyen2017ACL} & 92.58 & 91.91 & 91.50 & 90.73 & 91.74 & 90.47 & 90.61 & 91.36($\pm$0.14) \\
  Crowd-Cat~\citep{Nguyen2017ACL} & 92.71 & 91.71 & 92.48 & 91.15 & 92.35 & 91.97 & 91.22 & 91.94($\pm$0.08) \\
  Tri-Training~\citep{ruder-plank-2018-strong} & 92.84 & 92.15 & 92.51 & \underline{91.40} & 92.35 & 91.29 & 91.00 & 91.93($\pm$0.01) \\
  \midrule
  \textsc{ConNet} & \underline{92.97} & \underline{92.25} & \underline{93.15} & 91.06 & \underline{92.52} & \textbf{92.74} & \underline{91.66} & \underline{92.33}($\pm$0.17) \\
  \midrule
  Gold (Upper Bound) & 92.64 & 93.10 & 93.15 & 91.33 & 93.09 & 94.67 & 92.20 & 92.88($\pm$0.14) \\
  %Consensus Network + BEA & 92.83 & 92.18 & 92.31 & 91.15 & 91.81 & 92.03 & 91.18 & 91.93($\pm$0.15) \\
  \bottomrule
\end{tabularx}
}
\scalebox{0.76}{
\begin{tabularx}{1.3\textwidth}{l|X c X c X c X c X c X c X|l}
  \toprule
  Task \& Corpus & \multicolumn{14}{c}{\bf Multi-Domain NER: OntoNotes v5.0 - English} \\
  \midrule
  Target Domain & & nw & & wb & & bn & & tc & & bc & & mz & & AVG $F_1$(\%) \\
  \midrule
  CONCAT & & 68.23 & & 32.96 & & 77.25 & & \underline{53.66} & & 72.74 & & 62.61 & & 61.24($\pm$0.92) \\
  MTL-MVT~\citep{Wang2018BioNER} & & 65.74 & & 33.25 & & 76.80 & & 53.16 & & 69.77 & & 63.91 & & 60.44($\pm$0.45) \\
  MTL-BEA~\citep{rahimi2019massively} & & 58.33 & & 32.62 & & 72.47 & & 47.83 & & 48.99 & & 52.68 & & 52.15($\pm$0.58) \\
  \midrule
  Crowd-Add~\citep{Nguyen2017ACL} & & 45.76 & & 32.51 & & 50.01 & & 26.47 & & 52.94 & & 28.12 & & 39.30($\pm$4.44) \\
  Crowd-Cat~\citep{Nguyen2017ACL} & & 68.95 & & 32.61 & & 78.07 & & 53.41 & & \textbf{74.22} & & 65.55 & & 62.14($\pm$0.89) \\
  Tri-Training~\citep{ruder-plank-2018-strong} & & 69.68 & & 33.41 & & 79.62 & & 47.91 & & 70.85 & & 68.53 & & 61.67($\pm$0.31) \\
  \midrule
  \textsc{ConNet} & & \textbf{71.31} & & \textbf{34.06} & & \underline{79.66} & & 52.72 & & 71.47 & & \textbf{70.71} & & \textbf{63.32}($\pm$0.81) \\
  \midrule
  Gold (Upper Bound) & & 84.70 & & 46.98 & & 83.77 & & 52.57 & & 73.05 & & 70.58 & & 68.61($\pm$0.64) \\
  %Consensus Network + BEA & & 66.26 & & 33.21 & & 78.03 & & \textbf{55.74} & & 69.50 & & 68.76 & & 61.92($\pm$0.74) \\
  \bottomrule
\end{tabularx}
}
\scalebox{0.76}{
\begin{tabularx}{1.3\textwidth}{l|X c X c X c X c X|l}
  \toprule
  Task \& Corpus & \multicolumn{10}{c}{\bf Multi-Domain Text Classification: MDS} \\
  \midrule
  Target Domain & & books & & dvd & & electronics & & kitchen & & AVG $Acc$(\%) \\
  \midrule
  CONCAT & & 75.68 & & 77.02 & & 81.87 & & 83.07 & & 79.41($\pm$0.02) \\
  MTL-MVT~\citep{Wang2018BioNER} & & 74.92 & & 74.43 & & 79.33 & & 81.47 & & 77.54($\pm$0.06) \\
  MTL-BEA~\citep{rahimi2019massively} & & 74.88 & & 74.60 & & 79.73 & & 82.82 & & 78.01($\pm$0.28) \\
  \midrule
  Crowd-Add~\citep{Nguyen2017ACL} & & 75.72 & & 77.35 & & 81.25 & & 82.90 & & 79.30($\pm$9.21) \\
  Crowd-Cat~\citep{Nguyen2017ACL} & & 76.45 & & 77.37 & & 81.22 & & 83.12 & & 79.54($\pm$0.25) \\
  Tri-Training~\citep{ruder-plank-2018-strong} & & 78.75 & & 78.45 & & 81.95 & & 83.17 & & 80.58($\pm$0.02) \\
  %\cite{ruder-plank-2018-strong}* & & 74.86 & & 78.14 & & 81.45 & & 82.14 & & 79.15(~~~~-~~~~~) \\
  \midrule
  \textsc{ConNet} & & \underline{77.58} & & \textbf{81.06} & & \textbf{84.12} & & \underline{83.45} & & \textbf{81.55}($\pm$0.04) \\
  \midrule
  Gold (Upper Bound) & & 78.78 & & 82.11 & & 86.21 & & 85.76 & & 83.22($\pm$0.19) \\
  %Consensus Network + BEA & & 74.95 & & 76.05 & & 80.15 & & 82.75 & & 78.48($\pm$0.25) \\
  \bottomrule
\end{tabularx}
}
\caption[]{\textbf{Performance on cross-domain adaptation.} The best score (except the Gold) in each column that is significantly ($p<0.05$) better than the second best is marked \textbf{bold}, while those are better but not significantly are \underline{underlined}. * means the results from the paper.
}
\label{tab:app:domain}
\end{table*}

The performance of each method on each task is shown in Tab.~\ref{tab:res:domain}. We report the accuracy for POS tagging and text classification, and report the chunk-level F1 score for NER. We can see that \textsc{ConNet} achieves the highest average score in all tasks. \texttt{MTL-MVT} is similar to our decoupling phase without the attention module, which performs much worse. It shows that naively doing unweighted voting does not work well. The attention can be viewed as implicitly doing weighted voting on the feature level. 
This demonstrates the importance of having such a module to assign weights to all domains based on the input sentence. The Tri-Training model trained on the concatenated training data from all sources performs worse than \textsc{ConNet}, which suggests that it is important to have a multi-task structure to model the difference among domains. 
We analyze the OntoNotes dataset to show that the attention scores generated by the model are meaningful.

\begin{figure}[htbp]
\centering
    \includegraphics[width=0.9\linewidth]{figures/exp/multidomain/Attention_heatmap.png}
\caption{Heatmap of averaged attention scores from each source domain to each target domain.}
\label{fig:exp:att_heatmap}
\end{figure}

We analyzed the attention scores generated by the attention module on the OntoNotes dataset. For each sentence in the target domain we collected the attention score of each source domain, and finally the attention scores are averaged for each source-target pair. Fig.~\ref{fig:exp:att_heatmap} shows all the source-to-target average attention scores. We can see that some domains can contribute to other related domains. For example, bn (broadcast news) and nw (newswire) are both about news and they contribute to each other; bn and bc (broadcast conversation) are both broadcast and bn contributes to bc; bn and nw both contributes to mz (magzine) probably because they are all about news; wb (web) and tc (telephone conversation) almost make no positive contribution to any other, which is reasonable because they are informal texts compared to others and they are not necessarily related to the other. Overall the attention scores can make some sense to human, and it suggests that the attention is meaningful and contributing to the model.

==> sections/table2_bak.tex <==
\begin{table*}[h!]
% \vspace{-0.5cm}
\centering
\scalebox{0.7}{
%\begin{tabularx}{1.3\textwidth}{l|>{\centering}X|>{\centering}X|>{\centering}X}
% \begin{tabularx}{1.1\textwidth}{l>{\centering}X>{\centering}X>{\centering}X}
%\begin{tabularx}{\textwidth}{lccc}
\begin{tabular}{lccccccc}
  \toprule
  %Methods & POS Tagging & Name Entity Recognition & Text Classification
  \textbf{Methods} & \textbf{POS Tagging} & \multicolumn{3}{c}{\textbf{NER}} & \multicolumn{3}{c}{\textbf{Text Classification}}
  \tabularnewline
  %Corpus & UD - GUM & OntoNotes - English & MDS \tabularnewline
  %\midrule
  %& Avg $Acc$(\%) & Avg F1(\%) & Avg $Acc$(\%) \tabularnewline
  \midrule
  %\cmidrule{2-4}
  {CONCAT-SLM} & 92.11($\pm$0.07) & 00.00(+0.00) & 00.00(+0.00) & 61.24($\pm$0.92) & 00.00(+0.00) & 00.00(+0.00) & 79.41($\pm$0.02) \tabularnewline
  {MTL-MVT}%~\citep{Wang2018BioNER} 
  & 90.73($\pm$0.29) & 50.80(+1.04) & 57.26(+0.21) & 60.44($\pm$0.45) & 00.00(+0.00) & 00.00(+0.00) & 77.54($\pm$0.06) \tabularnewline
  {MTL-BEA}%~\citep{rahimi2019massively} 
  & 91.71($\pm$0.06) & 00.00(+0.00) & 00.00(+0.00) & 52.15($\pm$0.58) & 00.00(+0.00) & 00.00(+0.00) & 78.01($\pm$0.28) \tabularnewline
  \midrule
  {Crowd-Add}%~\citep{Nguyen2017ACL} 
  & 91.36($\pm$0.14) & 00.00(+0.00) & 00.00(+0.00) & 39.30($\pm$4.44) & 00.00(+0.00) & 00.00(+0.00) & 79.30($\pm$9.21) \tabularnewline
  {Crowd-Cat}%~\citep{Nguyen2017ACL} 
  & 91.94($\pm$0.08) & 00.00(+0.00) & 00.00(+0.00) & 62.14($\pm$0.89) & 00.00(+0.00) & 00.00(+0.00) & 79.54($\pm$0.25) \tabularnewline
  {Tri-Training}%~\citep{ruder2018strong} 
  & 91.93($\pm$0.01) & 00.00(+0.00) & 00.00(+0.00) & 61.67($\pm$0.31) & 00.00(+0.00) & 00.00(+0.00) & 80.58($\pm$0.02) \tabularnewline
  %\cite{ruder2018strong}* & - & - & 79.15(~~~~-~~~~~) \tabularnewline
  \midrule
  \textsc{ConNet} (Ours) & \underline{\textbf{92.33}}($\pm$0.17) & 62.07(+1.26) & 68.52(+0.25) & \textbf{63.32}($\pm$0.81) & 00.00(+0.00) & 00.00(+0.00) & \textbf{81.55}($\pm$0.04) \tabularnewline
  \midrule
  Gold (Upper Bound) & 92.88($\pm$0.14) & 71.62(+1.20) & 67.86(+1.16) & 68.61($\pm$0.64) & 00.00(+0.00) & 00.00(+0.00) & 83.22($\pm$0.19) \tabularnewline
  \bottomrule 
\end{tabular}
}
\caption[]{\small\textbf{Performance on cross-domain adaptation.} The average score for all domains is reported for each task. The best score in each column that is significantly ($p<0.05$) better than the second-best is marked \textbf{bold}, while those are better but not significantly are \underline{underlined}. %* means the results of the paper.
Detailed results can be found in Appendix~\ref{sec:app:domain}.
}
\label{tab:res:domain}
\end{table*}
%\subsection{Performance on Simulated Crowd-sourcing Datasets}

